Graph-Structured Visual Imitation

We cast visual imitation as a visual correspondence problem. Our robotic agent is rewarded when its actions result in better matching of relative spatial configurations for corresponding visual entities detected in its workspace and teacher's demonstration. We build upon recent advances in Computer Vision,such as human finger keypoint detectors, object detectors trained on-the-fly with synthetic augmentations, and point detectors supervised by viewpoint changes and learn multiple visual entity detectors for each demonstration without human annotations or robot interactions. We empirically show the proposed factorized visual representations of entities and their spatial arrangements drive successful imitation of a variety of manipulation skills within minutes, using a single demonstration and without any environment instrumentation. It is robust to background clutter and can effectively generalize across environment variations between demonstrator and imitator, greatly outperforming unstructured non-factorized full-frame CNN encodings of previous works.

==> experiments_old.tex <==
\section{Experiments}
\label{sec:exp}

\begin{figure}
    \centering
    \begin{subfigure}[b]{.48\textwidth}
        \includegraphics[width=\textwidth]{figures/task_pushing.png}
        \caption{\textit{Pushing}}
        \label{fig:pushing}
        \vspace{4ex}
        \includegraphics[width=\textwidth]{figures/task_pouring.png}
        \caption{\textit{Pouring}}
        \label{fig:pouring}
    \end{subfigure}
    \begin{subfigure}[b]{.48\textwidth}
        \includegraphics[width=\textwidth]{figures/cost_plot_overview.png}
        \caption{\textit{Stacking} and cost comparison}
        \label{fig:rewardshaping}
    \end{subfigure}\qquad
\caption{\todo{lets only keep the right part of the figure}Examples of the imitation tasks we consider. (a): \textit{pushing}, (b): \textit{pouring} (c): \textit{stacking} and \textbf{cost comparison of the proposed \VEG cost function  and the TCN embedding cost \cite{Sermanet2017}.} The  \VEG based cost curves are highly discriminative of the imitation quality for the stacking task, in contrast to TCN. 
	Costs are scaled between $[0, 1]$ by dividing by the maximum absolute value of the respective feature space for visualization purposes. \texttt{correct\_end} is simply repeating the last frame of a successful imitation, showing our lost function serves well as an attractor towards the final goal configuration.}
\label{fig:task}
\end{figure}

We test our visual imitation framework on a Baxter robot. We consider the following tasks to imitate:
\begin{enumerate}
    \item \textbf{Pushing}: The robot needs to push an object while following  specific trajectories.
    \item \textbf{Stacking}: The robot needs to pick up an object, put it on top of another one and release the object.
    \item \textbf{Pouring}: the robot needs to pour liquid from one container into another.
\end{enumerate}
Examples for each of the tasks are shown in Figures \ref{fig:task}. For every task, we train corresponding object detectors using synthetic data augmentation and  point features using multi-view self-supervised feature learning. Note that both processes are fully automated and \textbf{do not require human demonstrations or robot interactions}. Rather,  a camera that is setup to move around the scene in a prerecorded fashion suffices. 

Our experiments aim to answer the following questions:

\begin{itemize}
    \item Can the proposed \VEG representation  drive successful skill imitation?
     \item How does our \VEG encoding compare against convolutional image encodings of previous work \cite{Sermanet2017}?
     \item How robust are \VEGs to variability in the objects' spatial configurations and background clutter?
     \item How well can 
     \VEGs generalize across objects with different  shapes and textures?
\end{itemize}



\paragraph{Baseline:} 
We compare our method   against time-contrastive networks (TCN) of Sermanet et al. \cite{Sermanet2017}. 
We are not aware of other instrumentation-free methods that have attempted single shot imitation of manipulation skills, without assuming extensive pre-training with random actions for model learning \cite{DBLP:journals/corr/NairCAIAML17}.   
%\paragraph{Baseline: time-contrastive image embedding learning}
TCN trains an image embedding network using a  triplet ranking loss  \cite{Hoffer2015} 
ensuring that temporally near pairs of frames are closer to one another in embedding space than any temporally distant pairs of frames. %so that RGB frames near in time have small embedding feature distances, and RGB frames far in time have large embedding feature distance. 
In this way, the feature extractor focuses on the \textit{dynamic} part of the demonstration video. 
%Specifically, they use a  triplet ranking loss as introduced in \cite{Hoffer2015}, ensuring that temporally near frames are closer to each other in embedding space than any temporally distant pair of frames. 
We implemented the TCN baseline  using the same architecture as in \cite{Sermanet2017}, which consists of an Inception-v3 model \cite{Szegedy2015}, pretrained on ImageNet, up to the “Mixed 5d” layer which is then followed by two convolutional layers, a spatial softmax layer and a fully-connected layer. The network finally outputs a 32-dimensional embedding vector for the input image. For each imitation task, we train a corresponding TCN using 10 video sequences, 5 human demonstrations and 5 robot executions while performing tasks with relevant objects and environment configuration, together with the human demonstration we provide for learning the policy with VEG. 
With respect to the policy learning with TCN, we use a cost function of the form 
$\alpha||\mb{z}_t-\mb{w}_t||_2^2+\beta\sqrt{\gamma+||\mb{z}_t-\mb{w}_t||_2^2}$, where we choose $\gamma=10^{-5}$, $\alpha=1.0$, and $\beta=0.001$. Here, $\mb{z}_t$ and $\mb{w}_t$ denote the state embedding at each time step for the imitation and demonstration, respectively.

%Our method does not require additional data as TCN does.  
While our method uses only a single human demonstration, 
it does require training  object detection and point-feature network (both the data synthesizing for the object detector and the data collection for the point-feature network are fully automated though). 
In order to have a fair comparison, we put same amount of  effort into data collection for training TCN. 



\subsection{Cost Shaping}
We evaluate the robustness of the proposed VEG-based cost function in Eq. \ref{eq:reward} to  background clutter and its discriminativeness in guiding correct visual imitation. In Figure \ref{fig:rewardshaping}, we consider a human demonstration of a stacking task and  various robot executions under different conditions. We then show a comparison of the corresponding cost curves for each robot execution with the human demonstration,  computed by the proposed \VEG based cost function and the baseline TCN \cite{Sermanet2017}  cost function. The horizontal axis denotes time and the  vertical axis denotes imitation cost. The proposed graph-based cost correctly identifies all correct executions, despite heavy background clutter in the 5th row, and correctly signals the wrong  imitation segments in 2nd and 3rd rows. In contrast, the TCN cost curves are non discriminative. 
%, and \textit{2)} discriminative enough for effective skill learning
%We compare the cost computed based on VEG and TCN on the \textit{stacking} task, while we provide a single demonstration and evaluate the resulted cost at each timestep for robot's execution under different conditions. The results are visualized in Figure \ref{fig:rewardshaping}. 
%We show in the top row the successful demonstration, followed by successful imitation carried out by the robot and their corresponding cost shaping curve. Note our VEG encoding, compared to TCN, provides much more informative cost signal for the correct imitation, and more robust under different variations, which 
Cost curves which are highly discriminative in case of both successful imitation and also failure cases are critical for effective policy learning, which we discuss right below.

%We supplied  four demonstrations for the following tasks:


%We test the proposed what-where relational graph (WWG) image encoding  for visual imitation learning. The average distance of corresponding visual entities constitute the per frame rewards $\RR^t$ of Eq. \ref{eq:reward}. 
%For training our 





%Specifically, we use the proposed what-where graph encoding in place of image general encoding function $\phi$ of Eq. \ref{eq:reward}. 




% \paragraph{Reward shaping for visual imitation}
% We compare WWG and TCN for reward shaping, namely, judging when two videos depict correct execution of a task, in Figure \ref{fig:rewardshaping}. In each of the subfigures we show in the top row the human demonstrating a task, then a correct or wrong execution, and then the perceptual similarity values for the corresponding time steps for WWG and TCN encoding. For visualizing the reward for wrong executions, we simply repeats the first frame of the correct one, to show a clearer structural trend in the reward shaping.

% Note the WWG encoding, compared to TCN, is more discriminative for the correct task execution when producing reward signals.

% Note how WWG is robust to the presence of distractors, %TCN cannot learn 

% \todo{+++}
% we show perceptual similarity 
% We record several human demonstrations   and train our method to  train time-contrastive embeddings embeddings. We compare those 

%For a comparison between frame-centric single-view \cite{Sermanet2017} and the proposed object-centric image encoding, we compare in Fig. \ref{fig:frobj} the reward value of Eq. \ref{eq:reward} as produced by the two feature functions, while using only the object appearance features and not cross-object distances in our proposed feature function. The task is defined by rotating a cylindrically shaped object around one of its principal axis. In Fig.  \ref{fig:frobj} first row we show the human demonstration, in the second row we show a correct robot imitation and in the third row we show a wrong behaviour. In both cases, the feature encoding was trained using a video sequence in which the tower was moved by a human.
% Note the object-centric appearance features, here involving the one object of interest (yellow tower), are more discriminative of the correct task execution. The object-centric features are also more attentive towards minor changes in appearance, such as how the robot is holding the object.
%*****
%\subsubsection{Ring Stacking}
%For purely translational tasks, such as stacking or moving objects, the object location features are often sufficient and adding appearance  features is not imperative for the success of the learner. As an example task, we perform an experiment of putting a ring on top of a cylindrical tower object as demonstrated by a human. We show in Fig. \ref{fig:cc} the reward curves for only the spatial arrangement features that generalize well across objects (blue to green ring) and across human and robot demonstrator. Establishing cross-object correspondences  thus permits strong generalization for free using such appearance agnostic features, that do not require immense amounts of data to be trained in order to forget the appearance of the original objects.   
%To verify the usefulness of the global features, we set up a toy experiment where the goal is to put a ring on a tower. While using purely visual features fails to recognize when the robot is placing the ring on the tower \todo{where is this shown??}, using global features provides a clear differentiation between the different end states as seen in figure \ref{fig:cc}. 



% We record using HTC Vive few human demonstrations in the Bullet Physics simulator \cite{bullet}. The demonstations depict basic pick and place tasks, as well as rotation tasks

\subsection{Policy Learning}



% We evaluate the suitability of our method for learning manipulation policies both on a real Rethink Robotics Baxter robot on the following tasks:
% \begin{enumerate}
% 	\item \textbf{Pushing}: The robot needs to learn how to push a toy to a desired location given a human demonstration, as seen in Fig \ref{fig:pushing}. 
% 	\item \textbf{Rotating}: The robot needs to learn how to rotate a toy to a desire orientation given a human demonstration, as seen in Fig \ref{fig:rotating}.
% \end{enumerate}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{new_figures/red_cube_final_successrate.png}
% 	\caption{ The robot learns to stack the block for both our method and the \textit{blob detector} baseline. It fails to do so for the \textit{TCN} baseline. Our method imitates the original trajectory more closely due to to higher precision of the trained object detector.}
% 	\label{fig:cube-pilqr}
% \end{figure}

% We evaluate the following architectures:
% \begin{enumerate}
% 	\item \textit{ours}: Our WWG reward learning
% 	\item \textit{TCN}: frame-centric TCN using RGB input trained on demonstration data 
% % 	\item \textit{blob detector}: off-the-shelf blob detector generating encodings the same way as for our method 
% \end{enumerate}\\



\paragraph{Implementation details:}
For each task, we provide the robot agent  with a single human demonstration to imitate. 
We run the experiment on a NVIDIA GTX 1080Ti GPU. The inference time of the entire VEG pipeline takes around 0.2s, allowing real-time position control. A fixed episode length of 30 steps is adopted for all experiments. We use the publicly available   implementation of PILQR in \cite{fzftm-gpsi-16} and sample eight trajectory rollouts per iteration before each policy update in training. The action space of the policy includes translational movement along \textit{x}, \textit{y}, and \textit{z} axes in the world frame, rotation of the robot's end-effector and a binary grasp/release action. Note that both \textit{pushing} and \textit{stacking} only require translational movement of objects, so we compute cost only based on the object nodes in our graph. The point level nodes are enabled for the \textit{pouring} task, since rotation is critical for pouring. We fix the weights $w$ for each edge type to the same value of 1.
Videos of the human demonstration and the robot's learning process are included in the supplementary materials.
%available on our project site\footnote{\url{https://msieb1.github.io/visual-entity-graphs}}.


\subsubsection{Pushing}
In this task, the robot needs to push the yellow octagon towards the purple ring following the trajectory showed by the demonstrator (Figure \ref{fig:pushing}). We evaluate three task variations:
\begin{itemize}
    \item %\textbf{straight-line} 
    Pushing the object following a straight line.
    \item %\textbf{straight-line-grasped} 
    Moving the yellow octagon along a straight line with it being always grasped.
    \item %\textbf{direction-change} 
    Pushing the yellow octagon along a trajectory with a sharp direction change of 90 degrees. Imitating such direction change requires the robot to change the point of contact with the object during pushing.
\end{itemize}

\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Task & object & \VEG & TCN \\ \hline
\multirow{2}{*}{straight-line} & yellow octagon & 5/5 & 1/5 \\ \cline{2-4} 
 & orange square & 4/5 & 0/5 \\ \hline
% \multirow{2}{*}{straight-line-grasping} & yellow octagon & Success & Failure \\ \cline{2-4} 
%  & orange square & Success & Failure \\ \hline
straight-line-grasped & yellow octagon & Success & Failure \\ \hline
% \multirow{2}{*}{direction-change} & yellow octagon & Success & Failure \\ \cline{2-4} 
%  & orange square & Success & Failure \\ \hline
direction-change & yellow octagon & Success & Failure \\  \hline
%  & orange square & Success & Failure \\ \hline
\end{tabular}
\caption{Success rates for the pushing tasks under different settings.}
\label{tab:push}
\end{table}

For straight-line pushing, we attempted imitation in two different environments,
%run PILQR for both 
one with a yellow octagon block, and one with a smaller orange square block  to evaluate the generalization capability of our graph-based framework across  objects with different geometries. We essentially use the object detector for the small orange square block in the second case, in place of the detector of the yellow octagon block. %(see supplementary materials for details),

In order to test  the robustness of \VEG to variations in the objects' spatial configurations, for the basic straight-line pushing task, we randomly perturb the starting configurations of all the objects and the robot's end-effector within a norm ball of diameter 6cm, and run the policy training 5 times for each object. With the VEG representation, the robot's policy converges after 6 iterations in all tasks. We consider the task solved if the robot is able to push the object  within 1cm of the desired target position. We report the success rate for each case in Table \ref{tab:push}. The robot successfully solves the task for all 5 runs for the original yellow octagon, and for 4 runs out of 5 for the smaller orange square, demonstrating robustness against perturbation in objects' spatial configuration and strong generalization over objects with novel geometries. TCN failed in almost all runs, and for simple straight-line pushing could not reach even a quarter to the target even with significantly more iterations.

For the straight-line-grasped task, the robot is forced to keep the gripper closed. Hence, the robot cannot simply hard-imitate the hand trajectory, but rather needs to follow a trajectory that differs from the human demonstrator to successfully solve the task. In this sense, the hand trajectory of the human serves as a weak guiding signal during the policy learning.

The robot solves both straight-line-grasped and direction-change pushing after 8 iterations of trajectory optimization. Note that we increased the hand edge weight $w$ to account for stronger guidance of the hand during the direction-change task. TCN fails to solve any of the tasks, and in general performs very poorly in tasks where the robot does not have continuous contact with the object.



\subsubsection{Stacking}
In this task, the robot needs to reach and grasp the yellow octagon, position it on top of the purple ring, and then release it, as shown in the 1st and 4th rows in Figure \ref{fig:rewardshaping}. As in our pushing experiments, we randomize the starting configurations of the scene and the robot, and evaluate our method on this augmented setup for stacking both yellow octagon and the orange square. We report the results in Table \ref{tab:stack}. \VEGs enables robust policy learning for the yellow octagon, and shows generalization towards objects with novel geometries that have not been observed during demonstration. Being flatter than the octagon, the orange square is much harder to  grasp, yet the robot is able to learn the skill successfully most of the times.

The TCN baseline %performs poorly because its use of image-level embedding 
is not able to learn a successful grasping action, which requires precise and coordinated end-effector movement. We then evaluate TCN in a simpler task: stacking an already-grasped yellow octagon (simple-stacking in Table \ref{tab:stack}). The TCN performs reasonably well on this task, demonstrating its ability to imitate smooth trajectories, but non-ability of learning fine-grained grasping actions. 
\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Task & object & \VEG & TCN \\ \hline
\multirow{2}{*}{stacking} & yellow octagon & 4/5 & 0/5 \\ \cline{2-4} 
 & orange square & 3/5 & 0/5 \\ \hline
simple-stacking & yellow octagon & 5/5 & 3/5 \\ \hline
\end{tabular}
\caption{Success rate for the stacking task for our method and baseline with different starting configurations.}
\label{tab:stack}
\end{table}
\subsubsection{Pouring}
In this task, the robot needs to simultaneously translate and rotate the yellow can to reach the desired orientation above the mug, as shown in 2nd row in Figure \ref{fig:pouring}.  Using the same pouring demonstration, we additionally evaluate generalizability of \VEGs by imitating using a novel object with a different shape and  texture (Figure \ref{fig:pouring} 3rd row). %, but learning from the same single demonstration. 

Trajectory optimization converges after 10 iterations, and solves the task successfully for all the objects. The TCN baseline is able to move the can along the trajectory, but fails to rotate it to the right configuration for successful pouring.
% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{new_figures/bowl_and_cube_final_successrate.png}
% 	\caption{\textbf{Average success rate of block-in-bowl task with occluders.} The robot learns to place the block into the bowl for both our method and the \textit{blob detector} baseline. It fails to do so for the \textit{TCN} baseline. Due to the  occlusions introduced into the setup, the \textit{blob detector} shows much more variance because the detections are further off with respect to the ground truth state compared to our trained object detector.}
% 	\label{fig:bowl-pilqr}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/rotating_cost.png}
%     \label{fig:rotating_demo}
%     \caption{Learning progress of the rotating task.}
%     \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{figures/rotating.png}
%     \label{fig:rotating_learn}
%     \caption{Initial and end state of human demonstration and robot's learned policy. }
%     \end{subfigure}
%     \caption{Learning curve of total costs and comparison between human demonstration and robot execution with learned policy.}
%     \label{fig:rotating}
% \end{figure}
% \begin{figure}
% \centering
%   \includegraphics[width=0.5\textwidth]{new_figures/occ.png}
% \caption{\textbf{Robustness of trained detector} The Mask R-CNN detector trained via data dreaming is robust to occlusions in the scene. If the object is not detected, the detector is finetuned on-the-fly with synthetic data created from detections of the previous frame.}
% \label{fig:occ}
% \end{figure}
%We set the episode length to 20 for this task. With respect to the policy learning, the robot attempted the task 15 times between each policy update. During each time step, the detector network generates bounding boxes and masks of the relevant objects in the scene. 
%The robot solves the task after only one iteration of PILQR, having been shown a single demonstration, as shown in Fig. \ref{fig:bowl-pilqr}. There, we see the average success rate over multiple tries with varied starting positions of both objects, randomly sampled within a 10 cm radius of the original demonstration position. \\
%\indent Because we include partial occlusions in the form of distractor objects and artificial blacking out of pixels, the performance of the \textit{blob detector} deteriorates, while the trained detector network still manages to solve the task robustly. The task was not solved using the \textit{TCN} baseline, which was trained on 100 views of the provided demonstration.




\paragraph{Discussion/Limitations:} Imitating the human hand critically improves performance during  reaching and grasping motions in human demonstrations, which cannot be easily inferred from any object motion. Our method relies on unoccluded areas of the scene, and there is no current attempt to keep track of occluded entities. 
%Rather,  (fully) occluded visual entities are dropped from the graph. This is particularly the case for pixel or object part entities that get occluded much more often than larger object-level entities. For pixel-level entities, we randomly re-sample 500 pixels in the object mask at each time step. This big number of entities ensures the reward signal is consistent across rollouts and time steps. 
In light of this, a clear avenue for future work is learning to track through occlusions, and use a temporal visual memory to extract the reward graph from, as opposed to relying on visual frames.  
Active vision can also be used both to undo occlusions during imitation, and to observe the demonstrator from the most convenient viewpoint for the imitator. 
Another limitation is the lack of any model information, which would much accelerate policy search. An interesting avenue for future work would be learning a model over motion of such visual entities, and use it as a prior for better exploration during policy search.




==> intro3old.tex <==
\section{Introduction}


%\todo{to mention that we like inductive biases}
Humans learn skills by watching other humans \cite{Kuniyoshi}. The ability to learn from observation ---called visual imitation \cite{pathakICLR18zeroshot} or third-person imitation \cite{DBLP:journals/corr/StadieAS17}---
%to be distinguished from kinesthetic teaching \cite{Akgun:2012:TKK:2157689.2157815}--- 
%has always been a much-desired goal for Artificial Intelligence as a means of quickly programming agents in an intuitive manner by non-roboticists, as opposed to hard-coding their behaviors by engineers.
has always been a much-desired goal in artificial intelligence as a means of quickly programming agents in an intuitive manner, as opposed to  hard-coding their behaviors. %It is much less used currently than kinesthetic demonstration, where the demonstrator takes over the robot end-effectors and directly demonstrate the desired task.
Visual imitation requires  fine-grained understanding of the demonstrator's visual scene and its changes over time. The imitator then will use its own embodiment and dynamics to cause a similar change in its own environment. 
%The agent then needs to use his own embodiment and dynamics to cause a similar change in her own environment.  
%The goal of a visual demonstration  is to change the state of the environment in a predictable manner. The goal of the imitated behaviour is to generate a similar state change of the environment, not solely to mimic the movements of the demonstrator exactly.  
%The embodiments of the human and the robot are different,  which means that the human's motions and dynamics  cannot be directly mapped to the robot's body. 
%This is not the case for exactly in case of imitating human dancing, where we are interested in imitating the human motion as opposed to bring about a desired change in the scene. 
%Moreover, the robot does not have access to the forces employed by the human to perform the task, solely to the  visual scene evolution. 
Visual imitation then boils down to  learning a visual similarity  function between the demonstrator's and imitator's environments, whose maximization---via the imitator's actions---would result in correct skill imitation. This similarity function determines  which aspects of the visual observations are relevant to reproducing the demonstrated  skill, i.e., it defines what to imitate and what to ignore \cite{Schaal_TCS_1999}. 


\begin{figure}[ht!]
\centering
  \includegraphics[width=\textwidth]{figures/graph_vis_new.png}

\caption{ \textbf{Graph-structured visual imitation.} 
\todo{we should make those 4 images into a 2X2 with time increasing in the vertical dimension.}
We show the visual entity graphs for a human demonstration and robot imitation for two timesteps. Corresponding nodes in the human demonstration (left) and robot imitation (right) share the same color. The graphs  are hierarchical. Edges exist between object,  robot and human hand nodes and point feature nodes, and are added and deleted dynamically over time based on motion saliency, as shown in the figure with solid and dashed lines, respectively. Our imitation reward function is determined by the  agreement of the relative spatial arrangements along  corresponding edges present in the two graphs.  Our graph representation is robust to viewpoint variation between demonstrator and executor, and can handle cluttered backgrounds. %Our graph is built hierarchically with nodes at two levels. 
%On the \textit{parent} level \todo{need to think about a better name}, nodes are associated with object-level entities and human hand / robot end-effector. We build the edges dynamically: at each timestep, we identify an anchor object (purple block in this case) based on motion attention. Reward function is computed from the edges connecting the anchor object and other nodes (solid lines), while ignoring the the other edges (dashed lines).
%On the \textit{child} level, we random sample points (pixels) within the mask of each objects dynamically at each step in the imitation and build child nodes rooted on their object-level parents, and then establish pixel-level correspondences between the demonstration and the imitation.
%Visual entities can be objects (), feature points on objects, finger and robot joints. Nodes in the demonstrator and robot \VEGs are in one-to-one  correspondence. The  reward function of trajectory optimization  penalizes disagreement of the pairwise spatial arrangements for corresponding nodes. The reward accounts for node entities that are in motion or are about to move in the video of the demonstrator, to focus the attention of the imitator in the essential part of the scene for each timestep.  % the human aThe visual entity correspondences between samples taken from human demonstration and robot's execution. Top row: object- and pixel-level correspondences with object at the same spatial configuration. Bottom row: object- and pixel-level correspondences with object at different spatial configurations.
}
\label{fig:intro}
\end{figure} 
%our work


We propose    hierarchical graph video representations, we call visual entity graphs (VEGs), where nodes represent visual entities (objects, parts or points) tracked in space and time,  and edges represent their relative 3D spatial arrangements. Our graphical image encoding is based on the simple observation that  \textbf{the appearance  of the scene, in some level of abstraction} (objects, parts or points) \textbf{ remains constant throughout a demonstration, but the spatial arrangements  of  entities change over time}---an observation which follows directly from  laws of Newtonian physics.  
The proposed visual entity graphs  capture such what-where decomposition:  nodes represent visual entities that are in one-to-one correspondence between the demonstrator and imitator environments  and persist over time, and edges represent their 3D arrangements  which may change over time.  Our imitation reward function measures matching of the relative spatial distances between corresponding node pairs (as shown in Figure \ref{fig:intro}) and  guides reinforcement learning of manipulation tasks from a single video demonstration  using only a handful of real-world interactions. 

%We consider a simple motion saliency  heuristic to dynamically add edges between node entities that are in motion in the demonstration video, and focus in this way the reward function to the relevant part of the demonstrator's scene.  
Visual imitation then boils down to discovering  corresponding visual entities (objects, parts, or points) between the demonstrator's and imitator's environments. This requires fine-grained visual understanding of both demonstrator's and imitator's  environments.  
The objects used by the demonstrator  are often  not included in  the labelled image or object  categories of ImageNet \cite{imagenet_cvpr09} or MS-COCO \cite{DBLP:journals/corr/LinMBHPRDZ14},  thus,  pre-trained object-detectors are often not   useful.  
%We achieve scene-conditioned fine-grained visual understanding by marrying three powerful  
We build upon recent human body keypoint detectors,   self-supervised cross-view visual feature learning, feature tranfer, and synthetic data augmentation for training visual detectors of objects and parts on-the-fly which can fire on corresponding visual patterns 
%to obtain 
%\textit{scene-conditioned visual entity detectors} which 
%establish correspondences 
between the demonstrator's and imitator's workspace, despite  differences in embodiment between the robot and the human, differences in occlusion patterns, and in robot-human body visual discrepancies (Figure \ref{fig:intro}). 
 %The  proposed visual entity detectors,  though they may not localize the target entities in \textit{all} possible contexts, they can effectively track the objects and parts through partial occlusions in the \textit{current} scene contexts of the imitator and demonstrator. 
 %Due to occlusions and dis-occlusions, different visual entities participate in the reward function in different frames. \todo{maybe not talk about occlusion here since we don't focus on this in experiment?}

%knowledge transfer for visual imitation

 



Previous works in visual imitation either design a  similarity function to contain object 3D locations and 3D poses \cite{DBLP:journals/corr/abs-1709-10087} which they obtain from special instrumentation of the environment, such as AR tags  \cite{DBLP:journals/corr/KroemerS16}, or learn full image or image sequence convolutional image embeddings using  time-contrastive losses \cite{Sermanet2017,dwibedi2018learning}, frame prediction \cite{}, or other self (un)-supervised losses \cite{}. However, the data used to train such image embeddings are both human video demonstrations as well as  robot executions of the task, or parts of the task, so that the neural network embedding  function learns to be robust to the presence of the robotic gripper or human hand. Yet, the requirement of the robot executing the task beats the purpose of visual imitation, and brings it closer to kinesthetic teaching. The same holds for recent work of \cite{DBLP:journals/corr/abs-1806-09655}, which learns an image encoding via frame prediction using robot's execution data, albeit the paper title.  By construction, our proposed part-based graph representations can effectively ignore background clutter or irrelevant parts of the scene \cite{} by not including the corresponding nodes in the VEGs. Moreover, our visual entity detectors can effectively generalize across changes of object locations and poses, as we empirically demonstrate.  %can match entities  
%We empirically show our graph-based representations generalize better across re-arrangements of a scene, and are robust to background clutter. 
Instead, full-frame encodings of previous works \cite{Sermanet2017,DBLP:journals/corr/NairCAIAML17} that do not use a part-based decomposition during matching require a very large number of video examples of humans and robots executing the task to acquire similar generalization properties. 
%By examples, we mean videos of humans and robots executing the task, which is data hard to collect. 
They fail to imitate the demonstrated skill most of the times, as we show in our experiments. When humans imitate fellow humans, they are equipped with excellent  visual detectors, visual feature extractors, and motion estimators as opposed to learning those from scratch for every new task. 
We opt for a similar transfer of machine vision knowledge during imitation for robotic agents. 



%He is equipped with state-of-the-art human body and finger joint detectors and object / part detectors trained on-the-fly  using synthetic data dreaming or cross-view associations. 


We test our visual imitation method  on a Baxter robot on three tasks: \textit{stacking}, \textit{pushing} and \textit{pouring}. We show our agent   learns to imitate a demonstrated skill from a \textit{single} video demonstration.  In summary, our contributions are as follows:
\begin{enumerate}
    \item We capitalize over state-of-the-art 
    computer vision architectures and self-supervision techniques
   % human keypoint detectors, self-supervised feature learning \cite{florencemanuelli2018dense}, and on-the-fly synthetic data augmentation and generation 
   to drive imitation of human manipulation skills. % by tracking visual entities in demonstrator's and imitator's environments. 
   To the best of our knowledge, this is the first work that uses human finger visual detectors as opposed to environment instrumentation \cite{Schmidt2015} to track the demonstrator's hand for visual imitation learning of object manipulations.
    
    
    %\item We use motion saliency to guide attention to different  visual entities, and thus, make the proposed cost function focus on relevant visual entities. 
    
    \item We imitate using a single demonstration, without any robot random exploration as in \cite{DBLP:journals/corr/NairCAIAML17,pathakICLR18zeroshot}, or any data of the robot performing the task as in \cite{Sermanet2017}. We do so without ever having access to expert actions. %  while still handling long and structured tasks.
    
    \item We show imitation results on a real robotic platform. %, in contrast to previous works \cite{DBLP:journals/corr/StadieAS17}. 
\end{enumerate}
Our code and data will be made publicly available.
%While such background knowledge in \cite{DBLP:journals/corr/AgrawalNAML16,DBLP:journals/corr/NairCAIAML17} is provided to the agent in the form of forward and inverse models acquire with random exploration in similar scene to the one to imitate, here we supply it in the form of advanced fine-grained machine perception tools. 

\begin{comment}


Direct matching of pixel intensities is not a meaningful measure of  similarity \cite{DBLP:journals/corr/JohnsonAL16} as it is easily spoiled by difference in viewpoints, human body versus robot body parts, illumination changes, changes in object poses, etc.. 
Numerous previous works manually 
Few recent works attempt instead to   \textit{learn}  such visual similarity by training  image (or short image sequence) feature  embedding in which L2 distances capture the desired notion of similarity , use unsupervised time-contrastive losses where  %  that captures the desired notion of similarity, %as opposed to manually design it, using convolutional networks  and self-supervised objectives. 
%For example, Nair et al.  \cite{DBLP:journals/corr/NairCAIAML17} train  inverse and forward visual models, Sermanet et al. \cite{Sermanet2017}  employ   multi-view time-contrastive losses to train image embedding functions so that near-in-time  image frames have small embedding distance,  
far-in-time image frames have high embedding distances, images across different views of the same time instance also have small embedding distance. 
%``pull together" image encodings of nearby frames across different views and ``push apart" image encodings of far  in time frames. 
\end{comment}










==> model_new_old.tex <==


% \section{Visual Entity Graphs for Visual Imitation}



%Given a video demonstration and the initial state of the robot's environment, we 
%Our graph is built hierarchically with nodes at two levels, as illustrated in \ref{fig:intro}. On the \textit{object} level \todo{need to have a better name?}, nodes are associated with object-level entities. We activate the edges in the graph dynamically: at each timestep, we identify an anchor object (purple block in this case) based on motion saliency, and enable the edges between the anchor (solid lines) and all other objects, whlie disabling all other edges (dashed lines). On the \textit{point} level, we random sample points (pixels) within the identified mask of each objects dynamically at each timestep. We connect these child nodes with corresponding object-level parents, and establish pixel-level correspondences between the demonstration and the imitation. Additionally, we treat the edges connected to the \textit{hand/end-effector} differently (marked as yellow lines), since strict following of hand trajectory of demonstrator is not always the desired behavior for the learner, due to mismatch between hand/gripper embodiment. Therefore, the anchor-hand edge is used merely to provide a guidance signal for skill learning and weighted differently.



\section{Formulation}

We encode a  demonstration video of length $T$  provided by the human expert and an imitation video of the same length $T$ provided by the imitator in terms of two graph sequences
$\GG_D^t=\{\VV^t_{D},\EE^t_{D}\}, t=1 \cdots T$ and $\GG_I^t=\{\VV^t_{I}, \EE^t_{I}\}, t=1 \cdots T$, respectively. We omit the subscript $D$ or $I$ when either it is clear from the context or it is not important to which workspace we are referring to. %, for clarity.  
%$\GG_D^t=\{\VV^t_{D, o},\EE^t_{D, o}, \VV^t_{D, p},\EE^t_{D, p}, \VV^t_{D, h},\EE^t_{D, h}\}, t=1 \cdots T$ and $\GG_I^t=\{\VV^t_{E, o}, \EE^t_{E, o},\VV^t_{E, p}, \EE^t_{E, p},  \VV^t_{E, h}, \EE^t_{E, h}\}, t=1 \cdots T$, 
A node $\VV^t_i$ corresponds to the $i$th visual entity and its respective 3D $(X,Y,Z)$ world coordinate $\mathbf{x}^t_i$, and an edge $\EE^{t}_{(i,j)}$ correspond to  a 3D spatial relation  between two node entities to be preserved during imitation.  We define a visual entity node $\VV^{t}_i$  to be any object, object part, or point that can be reliably detected  in the demonstrator's \textbf{and} imitator's work space. All nodes are in one-to-one correspondence between the demonstrator and imitator graph, as shown in Figure \ref{fig:intro}.   An entity can dynamically appear and disappear over time. We only require each entity associated with the demonstration sequence to have a corresponding entity in the imitation sequence. 

We consider three types of nodes: object nodes $\VV_o$, point nodes $\VV_p$, and hand/robot nodes $\VV_h$.
%correspond to \textit{object}, \textit{point}, and \textit{hand/end-effector} node entities, respectively.
An object node represent any rigid or non-rigid object that constitutes a separate physical entity in the world, while a point node represents any 3D  physical point on an object, as seen in Figure \ref{fig:intro}. Hand/robot nodes represent the human wrist 3D location, and the robotic gripper center 3D location. 
%manipulation agent in the scene.
We do not consider edges between point nodes. Rather,  each point node is connected only to the object node it is part of. In that sense, our graphs are hierarchical. 
 
Our cost function at each time step $t$ measures visual dissimilarity across the demonstrator and imitator graphs $\GG^t_D$ and $\GG^t_I$ in terms of relative spatial arrangements of corresponding entity pairs, as follows:

\begin{equation}
\label{eq:reward}
    \mathcal{C}(\GG^t_D,\GG^t_I)= \sum_{i,j, i <j}  w(\EE^t_{(i,j)}) \cdot  \atte(\EE^t_{(i,j)}) \cdot \Bigl\| \left( \mathbf{x}_{D,i}^{t}-\mathbf{x}_{D,j}^{t}\right)     - \left( \mathbf{x}_{I,i}^{t} - \mathbf{x}_{I,j}^{t}\right)\Bigr\|, 
\end{equation}
\begin{figure*}[!t]
\centering
  \includegraphics[width=1.0\textwidth]{figures/model_overview_highres.JPG}
\caption{\textbf{Detecting visual entities.}
%\todo{new great figure to match the caption}
We use human hand keypoint detectors, multi-viewpoint feature learning, and synthetic image generation for on-the-fly object detector training from only a few object mask examples. Using a manually designed mapping between the human hand and the robot, the visual entity detectors can effectively bridge the visual gap between demonstrator and imitator environment, are robust to background clutter, and generalize across different object instances. 
}
\label{fig:entities}
\end{figure*}
where $\atte(\EE^{t}_{(i,j)}) \in \{0,1\}$ is a binary   attention function that determines whether a particular edge is present depending on the motion of the corresponding nodes, and  $w(\EE^{t}_{(i,j)}) \in \mathbb{R}$ denotes edge weights. We tie weights across all edges of the same type, namely, object-hand edges, object-object edges and object-point edges, they are hyper-parameters of our framework and we set them them empirically. Learning to adjust those weights per task is an interesting and straightforward direction, yet it would require more interactions which we cannot afford in the real robot platform. We leave this for future work.
 %The cost function encodes the relative spatial arrangements in 3D between all entities for which the binary attention function $\atte{(\EE^{t}_{(i,j)})}$ is 1. % for the associated edge $\EE^{t}_{(i,j)}$. 

 %, except for the  pushing through a 90 degree angled trajectory, in which we increased. %In the pushing task
%We use different weights for object-point edges and object-object edges. %, as detailed 
%$pa(\cdot)$ in the superscript maps a point node to its parent object node, and $\alpha$ and $\beta$ are weights to balance the cost, which in our case are simply used to average the cost over all corresponding nodes. The coordinate feature of the \text{hand/end-effector} entity is also weighted by $\lambda$, as mentioned earlier.




\subsection{Detecting Visual Entities} 

We define a visual entity to be any object, object part, or point that can be reliably detected in the demonstrator's and imitator's workspace.  
% 
 %Object detectors trained on the MS-COCO dataset \cite{Lin2014} are unsuitable since many objects the robot encounters  are not contained in the MS-COCO annotations and are thus unknown to the pretrained detector. 
 For imitating fine-grained manipulation of an object, inferring the translation of its bounding  box is not enough, rather, the object's 3D pose and deformation needs to be inferred and imitated. 
 %Moreover,  solely the translation of  an object's bounding box is insufficient for its fine-grained manipulation. Rather, an object's 3D pose and deformation needs to be inferred and imitated. 
 A central  design choice in our work is using point feature detectors and motion of the detected points to infer the object's change of pose between demonstrator's and imitator's environments, without additional learning, as opposed to training object appearance features extracted within the object's bounding box to encode object change pose or deformation. We opt for what-where decomposition of the object's appearance, as opposed to whole object box  embedding learning. %, we opt for   %rotation or deformation. 
 %++
 
 
 We assume no access to  human annotations that would mark relevant corresponding entities across demonstrator's and imitator's environments. 
We instead train scene-specific object and point detectors for  entities that can be reliably recognized across  demonstrator's and imitator's workspaces, and    human hand keypoint detectors for tracking the human hand. %, multi-view self-supervised point feature detectors and synthetic data augmentation. We detail each one below.
\paragraph{Human hand detectors} 
%End-to-end approaches such as \cite{Li} rely on large amounts of data to train hand-to-robot correspondences, and are therefore prohibitive in few-shot learning scenarios. Instead, 
We rely on state-of-the-art hand detectors of Simon et al. \cite{simon2017hand} to detect human finger joints, and obtain their 3D locations using a D435 Intel RealSense RGB-D camera.   We rely on forward kinematics and a calibrated camera with respect to the robot’s coordinate frame to detect the  3D locations of the tips of the robot’s end-effector. We map the finger tips of a Baxter robot's parallel-jaw gripper to the demonstrator's thumb and index finger tips.  We detect grasp and release actions by thresholding the distance between the two finger tips of the human during the demonstration of the task. 

%We detail each of those ideas right below. Our agent is equipped with a camera and a depth sensor. He can thus propose object masks in his workspace using background subtraction. 

%\paragraph{Diverse category-agnostic object detection}
%We train object detectors in Visual Genome \cite{krishnavisualgenome} that contains 3000 object categories. The trained detectors are very good at proposing meaningful and diverse visual  entities, in terms of objects or object parts, that exhibit the basic principles of closure, saliency, convexity, etc., as shown in Figure \ref{fig:overview}. We use the proposed bounding  boxes as candidates for visual entities, for which we train visual entities using the method}.   


%We train 
%\todo{maybe rui to write this? and we should compare without training in VG}

\paragraph{Multi-view self-supervised point feature learning}
 An agent that has access to its egomotion and can observe a static scene from multiple views, can   infer visual correspondences across views through  triangulation \cite{hartley2003multiple}. We use these self-generated visual correspondences to drive visual metric learning of deep feature descriptors that are robust to  changes in the object pose or camera viewpoint, and can establish such correspondence in absence of triangulation \cite{florencemanuelli2018dense}.   
 %recover such correspondences in the absence of viewpoint information, namely, to learn deep feature descriptors of points that are robust to  changes in the object pose or camera viewpoint. %In our case, such points are pixels in 2D images taken by the cameras.
%\todo{Xian to write details here and an equation, notes: full frame multiview in TCN is too coarse to recover fine-grained details, only within instance supervision, but it has been shown the descriptors learnt to generalize cross-instance}
%The object detectors provide the spatial location of the objects of interest in the scene while we need correspondences at a lower level to infer local object-level transformation, such as orientation change and deformation. Pixel-level correspondences between the demonstration and robot's executions provide rich information of the object's spatial information. Pixels exist as the finest entities in the scene and are used as nodes at the lowest level of granularity in our graph. We follow the approach presented in \cite{florencemanuelli2018dense} to learn descriptors for pixel entities and compute pixel correspondences. 
We collect videos of the workspace of the robotic agent  fully automatically. 
We use an RGB-D camera attached to the robot's end-effector and move the camera while following random trajectories that cover many viewpoints of the scene and at various distances from the objects. We use the robot's forward kinematics model to estimate the camera poses via hand-eye calibration, which, in combination with the known intrinsic parameters and aligned depth images, allows for robust 3D-reconstruction of the scene, and provides accurate pixel correspondences across different view points. The complete feature learning setup is illustrated in Figure \ref{fig:entities}. During training, we randomly sample image pairs from the video, and generate a number of matching and non-matching pixel pairs. We then minimize pixel-wise contrastive loss \cite{schmidt2017self, choy2016universal}, which forces matching pixels to be close in the learned feature spaces, while maintaining a distance margin for non-matching pixels. This point feature learning pipeline produces a mapping from an RGB image to dense per-point descriptors. 
Though supervision comes always from within-instance correspondences, the hope is the resulting feature descriptors to match across object instances, due to the limited capacity of the network model. We show that indeed this is the case in Figure \ref{fig:pouring}. 

% with the same resolution, and minimize the distance between matching pixels in the descriptor space, while enforcing at least a certain distance threshold for non-matching pixels.
%\todo{explain pixel feature generalizes over objects}

%Note that such metric learning for obtaining point features is performed given only within-instance correspondences, but within each class, generalization across different objects with different geometries and textures comes freely since learning such embedding are expected due the limited VC dimension of the network model. This enables our VEG representation with powerful generalizabilty to learn skills even with objects unseen in the demonstration.

% While such metric learning for pixel features occurs only over correspondences within the same object, generalization across objects of different geometries and textures in the same class comes freely. \todo{backed up citation?}This is because such embeddings are expected due to the limited VC dimension of the model. Our VEG representation is thus endowed with powerful generalizability that allows it to imitate tasks even with objects unseen in the demonstration. 

\paragraph{Synthetic data augmentation}

We use background subtraction to propose object masks, and train a
%\todo{max-some massage of humanoids}
%Using entity masks proposed by background subtraction and entity boxes  proposed by our category agnostic detector, we train
visual  detector  for each mask  using synthetic data augmentation, as shown in Figure \ref{fig:entities}.   %similar, to \cite{Sieb2019a}. %We use the  state-of-the-art deep visual detector architecture of Mask R-CNN \cite{DBLP:journals/corr/HeGDG17}. 
%We create synthetic data by rotating, translating and random-cropping the image, as well as  pasting  random object masks, and recovering the groundtruth (box or mask or point correspondence) with out detector or metric learner. 
Specifically, we create a large synthetic dataset by translating, scaling,  rotating and changing the pixel intensity of the extracted RGB masks. The segmented object masks often partially overlap with each other in the synthetic images. These overlaps are beneficial as they help the agent learn to detect amodal object boxes under partial occlusions. Since we generate such images, we  automatically know the groundtruth bounding box and mask that correspond to each object in each image.  We then finetune a Mask R-CNN object detector \cite{DBLP:journals/corr/HeGDG17}---initialized from weights learnt under the object detection and segmentation task in MS-COCO---to predict boxes and masks for the synthetically generated images. 
 




\subsection{Motion saliency for dynamic VEGs}

A demonstrator's environment may contain  objects that do not  participate in the demonstrating task. %It is believed that humans use simple motion heuristics to attend to the right part of a demonstration \cite{} when imitating others. \todo{+++}
We use similar motion saliency heuristics to dynamically over time decide what edges $(i,j)$ to consider in our imitation cost function of Eq. \ref{eq:reward}, we setting  $\atte{(\EE^{t,(i,j)})}=1$ to denote edge presence. 
We define an anchor object to be any object in motion, and in the case of no moving objects---e.g., when the demonstrator is simply reaching towards an object---we define the anchor box to be the  moving object in the near future.   
We consider edges between the anchor object node and all other object nodes in the scene, as well as the hand/robot node, and all point nodes that belong to the anchor object.
%, i.e. $\atte{(\EE^{t,(i,j)})}=1$, for all edges
% Such anchor-centric graph structure allows flexible camera viewpoint and is robust against shift in absolution spatial configurations of the objects \todo{what does this mean}.\\
This type of motion attention is a well-established principle that drives human attention during imitation. Work of \cite{Lee2009} uses AR markers to estimate such task relevance based on motion attention. We  simply use our object detection network to track objects in time to infer movement between the different objects in the scene. 


\subsection{Policy Learning with Visual Entity Graphs}

Our goal is the robot to imitate the intended object manipulation task from a single human visual demonstration. 
We formulate this as a reinforcement learning problem, where at each time step the cost is given by  Eq. \ref{eq:reward}. 
We use PILQR \cite{Chebotar2017} to minimize the cost function in Eq. \ref{eq:reward}, a state-of-the-art trajectory optimization method that combines a model-based linear quadratic regulator with path integral policy search  to better handle non-linear dynamics. %, which are in general scenarios vanilla LQR-based approaches struggle with. % PILQR is a state-of-the-art reinforcement learning algorithm that combines, in a principled manner, the model-based generalization of linear quadratic regulators together with path integral policy search's flexibility and ability to handle non-linear dynamics. 
%policy search reinforcement learning. The reinforcement learning is used to demonstrate that the learned rewards can be employed to acquire suitable manipulation policies. 
We learn a  time-dependent policy $\pi_t(\mathbf{u}|\mathbf{x};\theta)=\mathcal{N}(\mathbf{K}_t\mathbf{x}_t+\mathbf{k}_t, \mathbf{\Sigma}_t)$  
, where the time-dependent control gains are learned by alternating model-based and model-free updates, where the dynamical model $p(\mathbf{x}_t|,\mathbf{x}_{t-1},\mathbf{u}_t)$ of the \textit{a priori} unknown dynamics is learned during training time. 
The actions $\mathbf{u}$ are defined as the changes in the robot end-effector's 3D position and orientation about the vertical axis, giving a 4-dimensional action space. The state representation for  PILQR  consists of the joint angles, end-effector position, and the graph configuration of the scene, concatenated into one vector. For $N$ objects, this featurization scheme results in a $3+n_{joints}+\sum_{i=1}^{N_{anchors}}(N_{total}-1)*3+\sum_{i=1}^{N_{anchors}} dim(\phi)$ dimensional state space, where $n_{joints}$ denotes the number of joints of the robot and $\phi$ encodes the chosen node feature for a visual entity in the graph. In our case, we perform uniform sampling of pixels at each time step, and we directly incorporate the averaged pairwise distance of all pixels across demonstration and imitation into the state space, yielding $dim(\phi)=1$.
We further use behavioral cloning to infer opening and closing of the robot gripper by thresholding the distance between the human index finger and thumb during the demonstration. 



% For $N$ objects, this featurization scheme results in an $n_{joints}+(N-1)\times3+\sum_i dim(\phi_i)$ dimensional state space, where $n_{joints}$ denotes the number of joints of the robot and $\phi_i$ encodes the chosen node feature for every visual entity in the graph.  %We recommend using lower-dimensional local features when working with more objects.
%to learn the policy parameters $\theta$ in order to maximize the expected reward, although other policy search methods could also be applied .

%The resulting algorithm learns policies from few samples and it is well-suited for contact-rich manipulation skills. 



==> relatedold.tex <==
\section{Related  Work} \label{sec:related}




%Previous works in visual imitation either design a  similarity function to contain object 3D locations and 3D poses \cite{DBLP:journals/corr/abs-1709-10087} which they obtain from special instrumentation of the environment, such as AR tags  \cite{DBLP:journals/corr/KroemerS16}, or learn full image or image sequence convolutional image embeddings using  time-contrastive losses \cite{Sermanet2017,dwibedi2018learning}, frame prediction \cite{}, or other self (un)-supervised losses \cite{}. 

%However, the data used to train such image embeddings are both human video demonstrations as well as  robot executions of the task, or parts of the task, so that the neural network embedding  function learns to be robust to the presence of the robotic gripper or human hand. Yet, the requirement of the robot executing the task beats the purpose of visual imitation, and brings it closer to kinesthetic teaching. The same holds for recent work of \cite{DBLP:journals/corr/abs-1806-09655}, which learns an image encoding via frame prediction using robot's execution data, albeit the paper title.  By construction, our proposed  graph representations can effectively ignore background clutter or irrelevant parts of the scene \cite{} by not including the corresponding nodes in the VEGs. Moreover, our visual entity detectors can effectively generalize across changes of object locations and poses, as we empirically demonstrate.  %can match entities  
%We empirically show our graph-based representations generalize better across re-arrangements of a scene, and are robust to background clutter. 
%Instead, full-frame encodings of previous works \cite{Sermanet2017,DBLP:journals/corr/NairCAIAML17} that do not use a part-based decomposition during matching require a very large number of video examples of humans and robots executing the task to acquire similar generalization properties. 
%By examples, we mean videos of humans and robots executing the task, which is data hard to collect. 
%They fail to imitate the demonstrated skill most of the times, as we show in our experiments. When humans imitate fellow humans, they are equipped with excellent  visual detectors, visual feature extractors, and motion estimators as opposed to learning those from scratch for every new task. 
%We opt for a similar transfer of machine vision knowledge during imitation for robotic agents. 


\paragraph{Visual imitation learning}
Imitation learning  addresses  
the problem of learning skills by observing expert demonstrations, and is considered  an important topic in the field of robotics due to its potential to highly expedite trial-and-error learning  \cite{Schaal_TCS_1999}.  However, 
most previous approaches assume that expert demonstrations are given in the workspace of the agent, (e.g., through kinesthetic teaching or teleoperation  \cite{Hussein:2017:ILS:3071073.3054912,Argall:2009:SRL:1523530.1524008}) and the actions/decisions of the expert can be imitated directly, either with behavioral cloning (BC) \cite{DBLP:journals/corr/abs-1710-04615}, inverse reinforcement learning (IRL) \cite{Ng:2000:AIR:645529.657801}, or generative adversarial imitation learning (GAIL) \cite{NIPS2016_6391}.  

%\paragraph{Visual imitation}
Imitating humans based on visual information is  much more challenging  due to the difficult visual inference needed for fine-grained activity understanding \cite{DBLP:journals/corr/StadieAS17}. In this case, a mapping between observations in the demonstrator space to observations in the imitator space is required and is essential for successful imitation  \cite{Nehaniv:2002:CP:762896.762899}. 
% but, most importantly, inference of the ``reward", that is, goal of the behaviour, that the agent will attempt to match by self-practise.
Numerous works bypass the difficult perception problem by using special instrumentation of the environment, such as AR tags, to read off object and hand 3D locations and poses during video demonstrations, and use rewards based on known 3D object goal configurations \cite{DBLP:journals/corr/abs-1709-10087,DBLP:journals/corr/KroemerS16}.  %the need for special instrumentation  hinders scaling-up learning from demonstration.  
Other works  
%does not attempt to learn rewards for actions \cite{DBLP:journals/corr/RahmatizadehAB16},  
use hand-designed reward detectors that work only in restrictive scenarios \cite{MullingKKP2012_2}. 

%\paragraph{Perceptual reward learning}
Recent approaches attempt to mimic the demonstrator's behaviour by directly matching whole image feature embeddings, and avoid  explicit extraction of the scene structure in terms of objects and poses. 
%or learn full image or image sequence convolutional image embeddings using  time-contrastive losses \cite{Sermanet2017,dwibedi2018learning}, frame prediction \cite{}, or other self (un)-supervised losses \cite{}. 
%However, the data used to train such image embeddings are both human video demonstrations as well as  robot executions of the task, or parts of the task, so that the neural network embedding  function learns to be robust to the presence of the robotic gripper or human hand. Yet, the requirement of the robot executing the task beats the purpose of visual imitation, and brings it closer to kinesthetic teaching. The same holds for recent work of \cite{DBLP:journals/corr/abs-1806-09655}, which learns an image encoding via frame prediction using robot's execution data, albeit the paper title.  By construction, our proposed  graph representations can effectively ignore background clutter or irrelevant parts of the scene \cite{} by not including the corresponding nodes in the VEGs. Moreover, our visual entity detectors can effectively generalize across changes of object locations and poses, as we empirically demonstrate. 
Numerous objectives have been proposed to learn full image or image sequence convolutional image embeddings using  multiview invariant and time-contrastive losses \cite{Sermanet2017,dwibedi2018learning}, forward and inverse dynamics model learning in \cite{pathakICLR18zeroshot,DBLP:journals/corr/AgrawalNAML16}, or reconstruction and temporal prediction objectives in \cite{DBLP:journals/corr/FinnTDDLA15,DBLP:journals/corr/WatterSBR15}. Work of  \cite{DBLP:journals/corr/abs-1802-04181} provides an overview of common objectives and inductive biases for state representation learning. However, the data used to train such image embeddings are both human video demonstrations as well as  \textit{robot executions of the task}, or parts of the task, so that the neural network embedding  function learns to be robust to the presence of the robotic gripper or human hand. Yet, the requirement of the robot executing the task beats the purpose of visual imitation, and brings it closer to kinesthetic teaching. The same holds for recent work of \cite{DBLP:journals/corr/abs-1806-09655}, which learns an image encoding via frame prediction using robot's execution data, albeit the paper title. Instead, learning our graph video encoding does not require robot executions.


%A single RGB frame or an entire sequence of frames is encoded into an embedding vector using a combination of forward and inverse dynamics model learning in \cite{pathakICLR18zeroshot,DBLP:journals/corr/AgrawalNAML16},  multiview invariant and time-contrastive metric learning in \cite{Sermanet2017}, or reconstruction and temporal prediction objectives in \cite{DBLP:journals/corr/FinnTDDLA15,DBLP:journals/corr/WatterSBR15}.  Work of  \cite{DBLP:journals/corr/abs-1802-04181} provides an overview of common loss metrics and inductive biases for state representation learning. 

 %Having learnt a latent state feature space, imitation is carried out by iterative application of the inverse model in \cite{pathakICLR18zeroshot,DBLP:journals/corr/AgrawalNAML16}, or via trajectory optimization in  \cite{Sermanet2017}. 
%, where the state is the combination of the latent visual state embedding vector and the robot configuration.
%Similar to \cite{Sermanet2017}, we use a  trajectory optimization method \cite{Chebotar2017, theodorouAISTATS2010} to imitate a human visual demonstration. However, instead of learning  a convolutional neural network to embed an image into a single 1D feature  vector, we learn to detect salient objects and parts, and establish the matching of the relative distances of corresponding visual entities in 3D space in demonstrator's and learner's environments as a learning signal. % spatial arrangements. 

Similar to our work, work of \cite{Sieb2019a} also uses 3D spatial object arrangements to guide visual imitation of manipulation tasks. However, they do not consider human keypoints or any entities finer than objects, which suggests their method can only imitate simple translation tasks, where object pose is not relevant (e.g., they cannot handle rotation). %We additionally use human finger keypoint detectors and point-based image features to handle grasping and other fine-grained object manipulation tasks.
Work of \cite{TOGSFV} utilizes human pose detectors to imitate 3D human motion extracted from YouTube videos of acrobatic activities in simulation. However,  no contact with objects is considered, and  imitation of human motion only happens in a simulated agent.   
%, but demonstrations are limited to physically simulated humanoids and robots. 
In comparison, we do not imitate motion alone, but rather, we  carry out a desired manipulation of the environment. Human hands are part of the graph we attempt to create, but so are the surrounding objects in the scene. 



 \paragraph{Scene graphs, object-centric reinforcement learning, and relational neural networks}
 %\todo{this requires work}
 Representing a visual  observation in terms %nodes 
 %Utilizing graph encodings of a visual scene in terms 
 of objects or 
 parts and their pairwise relations has been found beneficial for generalization of action-conditioned scene dynamics  \cite{DBLP:journals/corr/KanskySMELLDSPG17,DBLP:journals/corr/FragkiadakiALM15, DBLPjournals/corr/BattagliaPLRK16},   body motion and person trajectory forecasting \cite{DBLP:journals/corr/JainZSS15,7780479}, and reinforcement learning \cite{Diuk:2008:ORE:1390156.1390187}. Such graph-encodings have also been used to learn a model of the agent \cite{graphnet}, and use it for model-predictive control in non-visual domains. Work of Devin et al. \cite{Devin2017} uses pretrained object detectors and learns attention over the obtained detection boxes, which are incorporated as part of the state representation for policy learning. The graph representation we propose in this work not only employs explicit attention  to relevant objects, parts, and points, but also preserves their correspondence in time, i.e., the detectors \textit{bind} with specific objects, parts, points over time. 

 
 %Many works use a spatial softmax layer in CNNs that explicitly attempts to find keypoint detectors whose spatial coordinates would be a useful encoding of the visual frame \cite{DBLP:journals/corr/FinnTDDLA15,DBLP:journals/corr/FinnTDDLA15}. Extensive training data is required to learn such keypoint detectors from demonstration data. The output of the spatial softmax has been used as a state representation, and has not been tried as a reward function for imitation. %between learner and teacher. %We argue %Tjhose works did not use obtained detectors  this as entities that correspond between imitator and executor. 
 %In  contrast to the work of \cite{DBLP:journals/corr/FinnTDDLA15} which learns to represent an RGB image in terms of spatial coordinates of few keypoints, 
 %we instead consider a variety of spatial entities using also knowledge of the agent acquire \textit{before imitation} as weights of a general object/part detector architecture, and multiview self-supervised objectives.
 
 %employ explicit attention only to relevant objects, and preserve their correspondence in time, i.e., the detectors \textit{bind} with specific objects in the scene. 
 


\begin{comment}
\paragraph{Synthetic data agumentation:}
Synthetic data augmentation showed to be very successful in various machine perception tasks \cite{Park2015ArticulatedPE,GhiasiYRF_CVPR_2014,DBLP:journals/corr/TobinFRSZA17,DBLP:journals/corr/SadeghiL16}. In \cite{GhiasiYRF_CVPR_2014}, images with cross-person occlusions are generated to help train occlusion-aware detectors. 
Context-specific data augmentation was used in \cite{DBLP:journals/corr/KhorevaBIBS17} to train neural networks for object video segmentation. The work of \cite{DBLP:journals/corr/TobinFRSZA17} showed that domain randomization, namely augmenting textures of the background and the objects, even in a non-visually plausible way,  helps in training successful detectors that work on real images. 
\end{comment}


%In \cite{}, 
%Similar language-drive object attention has been proposed in \cite{DBLP:journals/corr/abs-1804-10692}. Our work uses real world reinforcement learning as opposed to high sample complexity reinforcement learning in simulation-, object appearance features and pairwise relative locations as opposed to just bounding box coordinates, and we demonstrate how explicit attention is important for being robust to random distractors in the environment, as we demonstrate in our experiments. 
%we should add this line later





 
 %Many computer vision methods propose representing a visual scene in terms of the objects it contains and their cross-relationships, a representation also known as scene graph \cite{}. Such representation has been shown to be beneficial for downstream tasks, such as, image captioning \cite{} and image retrieval \cite{}. For learning scene dynamics,  encoding a visual scene in terms of objects and their relationships, and sharing the neural  weights of the future predictor across objects  has shown to generalize better across the number of objects present \cite{}.  Taking an object-centric representation one step further, relational networks used in \cite{} aggregate neural pairwise interactions across various object or agent part pairs for learning dynamics that exhibit good generalization properties \cite{}. Works of \cite{} learn to encode the visual scene in terms of keypoints and their spatial coordinates.  However, in the presence of similar objects or novel objects, though they can be irrelevant to the task in hand, the representation can fail, due to lack of explicit attention to the relevant objects in the scene. Work of \cite{} showed how an entity-centric encoding of the scene and entity attributes and learning of structured dynamics with explicit selection of the relevant pre-conditions, and model-predictive control using such dynamics for look-ahead, can better handle environmental changes, in comparison to frame-centric reinforcement learning. 
 %Graph representations have gained attention recently, as they are capable of carrying our relational reasoning  between entities for visual recognition \cite{}, question answering \cite{}, model learning and control \cite{}. Here we focus on a particular form of relational graphs where edge encoding \textit{where} relationships, namely, distances between the nodes. This is particularly convenient as learning is not required for computing such edge features, rather, can focus on learning nodes that correspond across the two scenes. 


